Cross-modal Contrastive Learning for Speech Translation

How can we learn unified representations for spoken utterances and their written text? Learning similar representations for semantically similar speech and text is important for speech translation. To this end, we propose ConST, a cross-modal contrastive learning method for end-to-end speech-to-text translation. We evaluate ConST and a variety of previous baselines on a popular benchmark MuST-C. Experiments show that the proposed ConST consistently outperforms the previous methods on, and achieves an average BLEU of 29.4. The analysis further verifies that ConST indeed closes the representation gap of different modalities -- its learned representation improves the accuracy of cross-modal speech-text retrieval from 4% to 88%. Code and models are available at https://github.com/ReneeYe/ConST.

==> 051_xstnet_drawback.tex <==

Although previous research~\cite{ye2021end} has obtained good speech translation metrics via shared Transformer sub-module and multi-task learning, 
there is still a gap between the text embedding and the acoustic representation of speech, which makes the utilization of pre-training inefficient during the fine-tuning phase.
In this section, we randomly select several sentences and their speeches from MuST-C En-De test set to examine how distinct the representations of the two modalities are.
Figure~\ref{fig:xstnet1.0_kde}(a) illustrates such gap in modal representations, which is plotted as follows:
For speech $\vecs$ with acoustic representation $\veca$ and its transcript $\vecx$ with embedding $\vece$, we first average them in terms of the time dimension, 
\begin{align}
    \mathcal{R}=\text{MeanPool}(\veca), &\mathcal{R} \in \mathbb{R}^d \label{eq:audio_emb}\\
    \mathcal{E}=\text{MeanPool}(\vece), &\mathcal{E} \in \mathbb{R}^d \label{eq:text_emb}
\end{align}
We then reduce both representations to two dimensions according to T-SNE~\citep{van2008visualizing}.
As the cases in Figure~\ref{fig:xstnet1.0_kde}(a), we find that the representations of speech and transcript corresponding to the same meaning are distant from each other.
In addition, the average cosine similarity of the two modal representations of the same meaning is 0.31, which does not indicate a strong positive correlation between them.
Figure~\ref{fig:xstnet1.0_kde}(b) shows the bi-variate kernel density estimation~\cite{parzen1962estimation} of the dim-reduced feature from $\mathcal{R}$ and $\mathcal{E}$.
Ideally, if the representations of speech and its corresponding transcription are similar, then their KDEs will be similar, and thus, the contour lines will overlap as much as possible.
However, Figure~\ref{fig:xstnet1.0_kde}(b) shows that the audio and transcript textual representations are so distinct that they are automatically separated into two clusters.



\begin{figure}
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \centering
    \subfigure[Case analysis]{
        \begin{minipage}{0.47\linewidth}
            \centering
            \includegraphics[scale=0.2]{Figures/stgap_sample.pdf}
        \end{minipage}
    }
    \subfigure[Bivariate KDE contours]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[scale=0.25]{Figures/baseline_emb_kde.pdf}
        \end{minipage}
    }
    \caption{\textbf{(a)}: The average-pooled audio representations and text embeddings of selected transcription.
    \textbf{(b)}: the bi-variate KDE contour plot of the representation of speech and transcript in source language English. T-SNE is used to reduce the dimension into two. The blue circle and lines are the audio representations and the red triangle and dashed lines stand for text.}
    \label{fig:xstnet1.0_kde}
\end{figure}

